Fairness in Online Social Network Timelines: Measurements, Models and Mechanism Design

Facebook News Feed personalization algorithm has a significant impact, on a daily basis, on the lifestyle, mood and opinion of millions of Internet users. Nonetheless, the behavior of such algorithm lacks transparency, motivating measurements, modeling and analysis in order to understand and improve its properties. In this paper, we propose a reproducible methodology encompassing measurements, an analytical model and a fairness-based News Feed design. The model leverages the versatility and analytical tractability of time-to-live (TTL) counters to capture the visibility and occupancy of publishers over a News Feed. Measurements are used to parameterize and to validate the expressive power of the proposed model. Then, we conduct a what-if analysis to assess the visibility and occupancy bias incurred by users against a baseline derived from the model. Our results indicate that a significant bias exists and it is more prominent at the top position of the News Feed. In addition, we find that the bias is non-negligible even for users that are deliberately set as neutral with respect to their political views, motivating the proposal of a novel and more transparent fairness-based News Feed design.

==> fifo.tex <==

\subsection{Filtered FIFO News Feed model}
First we will provide a model for the News Feed. We assume that posts enter and leave the News Feed following a chronological order in a first-in first out fashion (FIFO). The algorithm decides which posts will be admitted in the News Feed. We will refer this operation as a filtered FIFO News Feed model.
Our goal is to create a model to obtain the steady-state distribution of the visibility and occupancy of a given publisher in the News Feed of user $i$. 



Before presenting the model, we start by introducing the notation and concepts used in this work. All the variables used are summarized in Table \ref{tab:notation}. 

\begin{table}[h]
\centering
\begin{tabular}{l l}
%\vspace{+0.1 in}
\hline
\hline
Variable & description \\
\hline
$j$ & target publisher \\
$i$ & user News Feed \\
$\lambda_j$ & creation rate of publisher $j$\\
$p_l$ & selection probability for the class-$l$
\\
%$\lambda_{i,-j}$ & arrival rate of other publishers than $j$ at $i$\\
%$\mathbf{\lambda_i}$ & vector of arrival rates of all publishers at $i$\\
$\lambda_i$ & total arrival rate at user $i$\\
%$\Lambda_{(-j)}$ & total arrival rate of other publishers than $j$\\
%$\mu_i$ & mean timer rate for publisher $j$ contents\\
$T_l$ & expected TTL timer duration for class-$l$\\
$w_{l}$ & weight associated to class-$l$  \\
$h_{ij}$ & hit probability at $i$\\
$\hat{\pi}_{ij}^{(m)}$ & measured visibility of $j$ at $i$\\
$\pi_{ij}$ & model visibility \\
$N_{ij}^{(m)}$ & measured occupancy  of $j$ at $i$\\
$N_{ij}$ & model occupancy of $j$ at $i$\\
%$H_i^{(t)}$ & Entropy at snapshot (t)\\
%$R_i^{(t)}$ & Richness at snapshot (t)\\
%$p_{ij}$ & probability of selecting a post from publisher $j%$ to \\
% & fill a given slot of News Feed of user $i$\\
%$T_j(k)$ & expected busy period when publisher $j$ enter the News Feed in position k \\
%$N$ & contents viewed per snapshot \\
%$w_j$ & weight associated to publisher $j$\\
%$\Omega$ & function domain \\


%$p_{il}$ & probability of a content from publisher $i$ has size $l$ \\
%$b_i,u_i,v_i$ & weights associated to publisher $j$\\
%$C$ & cost function \\
%$\phi$ & maximum publishing rate \\
%$\gamma$ & balance term in cost funtion\\
%$F^{(n)}$ & value of function $F$ at the n-th iteration\\ 
%$q_j$ & price for publisher $j$\\ 
%$S_j$ & desired setpoint of a metric of publisher $j$\\

\hline

\end{tabular}
\caption{Table of Notation}
\label{tab:notation}
\end{table}


Although every user in the Facebook has the possibility to 
produce posts, we have clear delineation between users and publishers. Thus, we characterize the 
publisher-user interaction as a bipartite graph, with $\mathcal{I}:=\{1, \dots,i,\dots I\}$ the set of users and $\mathcal{J}:=\{1, \dots,j,\dots J\}$ the set of publishers. 

Let $\mathcal{J}_i:=\{1,\dots,j,\dots J\}$ be the set of publishers followed by user $i$.  
Publisher $j$ creates and publishes posts according to a Poisson process with rate $\lambda_j$. Let $l:=\{0,1\}$ be the class that a publisher can belong. The class-$0$ is reserved for the preferred publishers, and the class-1 is reserved for the residual publishers.   A post from publisher $j$ belonging to the class-$l$ is selected to appear in the News Feed with probability $p_l$. Therefore, the effective arrival rate of posts of publisher $j$ at news feed of $i$ is equal to $p_l\lambda_j$.
Define the total rate of contents arriving at the news feed as:
\begin{equation}
\Lambda_i=\sum_{j=1}^J p_l\lambda_{j}
\end{equation} 


Define further the arrival rate of other publishers than $j$ :

\begin{equation}
\Lambda_{i,-j}= \Lambda_i-p_l\lambda_{j}
\end{equation} 

Figure \ref{fig:News Feed_schema} shows a schematic model for a news feed. Assume that a new post enters at the top of the news feed at position 1. With rate $\lambda_i$, posts arrival at position 1 shifting older contents to higher positions. Assume that a news feed has finite size of $K$ slots. A post is evicted from news feed if it is shifted from position $K$ to the fictitious $K+1$ slot by a new post.

\begin{figure}
\begin{center}
\includegraphics[scale=0.5]{Fifo_Timeline_single_size.eps}
\end{center}
\caption{Schematic model for news feed of user $i$ }
\label{fig:News Feed_schema}
\end{figure}

\begin{figure}
\begin{center}
\includegraphics[scale=0.6]{Markov_chain.eps}
\end{center}
\caption{CTMC for the topmost position of a post from publisher $j$ at news feed of user i }
\label{fig:CTMC}
\end{figure}

Figure \ref{fig:CTMC} shows a continuous time Markov chain (CMTC) whose state variable $X$ is the topmost position of publisher $j$. Let $\tilde{\pi}_x=P[X=x]$. Note that in a news feed a publisher may have more than one post simultaneously, but we account only for the slot of the most recent post of $j$. With rate $\lambda\pubj$, a post from publisher $j$ arrives at the top of news feed.  With rate $\lambda_{i,-j}$, a post from other publisher than $j$ shifts down publisher $j$. Publisher $j$ is out of news feed when it is position $K+1$, therefore, the visibility $\pi_{ij}$ is equal to $1-\pi_{K+1}$. Now we are able to state the following proposition 

\begin{proposition}
\[\pi_{ij}= 1-\bigg(\frac{\Lambda_{i,-j}}{\Lambda_i}\bigg)^K\]
\label{prop:fifo_newsfeed}
\end{proposition}




\begin{proof}
The balance equation for the steady-state probability  $\tilde{\pi}_1$ is

\begin{eqnarray}
\Lambda_{i,-j}\tilde{\pi}_1&=&\sum_{x=2}^{K+1} p_l\lambda_j \tilde{\pi}_x \\
&=&p_l\lambda_j (1-\tilde{\pi}_1)
\end{eqnarray}

Therefore, 

\begin{equation}
(\Lambda_{i,-j}+p_l\lambda_j) \tilde{\pi}_1=p_l\lambda_j
\end{equation}

Hence,
% * <e.hargreaves@gmail.com> 2018-05-05T14:43:15.876Z:
%
% ^.

\begin{equation}
\tilde{\pi}_1=\frac{p_l\lambda_j}{\Lambda_i}
\end{equation}

For state $x=2$ the balance equation is:

\begin{equation}
(\Lambda_{i,-j} + p_l\lambda_j)\tilde{\pi}_2= \Lambda_{i,-j} \tilde{\pi}_1
\end{equation} 

\begin{eqnarray}
\tilde{\pi}_2&=&	\frac{\Lambda_{i,-j}}{\Lambda_i}\tilde{\pi}_1 \\
&=&	\frac{\Lambda_{i,-j}}{\Lambda_i}\frac{p_l\lambda_j}{\Lambda_i}
\end{eqnarray}

It is straightforward to check that for a state $x$ in the interval $(1,K+1)$, the balance equation is:

\begin{equation}
\tilde{\pi}_x=\bigg(\frac{\Lambda_{i,-j}}{\Lambda_i}\bigg)^{x-1} \frac{p_l\lambda_j}{\Lambda_i}
\end{equation}

For state $x=K+1$, the balance equation is:

\begin{eqnarray}
\Lambda_{i,-j} \tilde{\pi}_K &=& p_l\lambda_j\tilde{\pi}_{K+1}\\
\tilde{\pi}_{K+1}&=& \frac{\Lambda_{i,-j}}{p_l\lambda_j} \tilde{\pi}_K \\
&=&\frac{\Lambda_{i,-j}}{p_l\lambda_j} \bigg(\frac{\Lambda_{i,-j}}{\Lambda_i}\bigg)^{K-1} \frac{p_l\lambda_j}{\Lambda_i} \\
&=&  \bigg(\frac{\Lambda_{i,-j}}{\Lambda_i}\bigg)^{K} 
\end{eqnarray}

Proposition \eqref{prop:fifo_newsfeed} follows because $\pi_{ij}=1-\tilde{\pi}_{K+1}$


\end{proof}

\begin{proposition}
\[N_{ij}= \frac{p_l\lambda_j K}{\Lambda_i}\]
\label{theo:occupancy_fifo}
\end{proposition}

\begin{proof}
Once the $m^{th}$ post enter in the news feed, it remains there  until the arrival of the $(m+K+1)^{th}$ post. Because the expected time between arrivals is $1/\Lambda_i$, the expected \textit{system time} of the $m^{th}$ post is $K/\Lambda_i$. Because we are interested in steady-state probabilities, $K/\Lambda_i$ is also the mean system time $T_{ij}$ of publisher $j$ at news feed $i$.  By \textit{Little's law}, 

\begin{eqnarray}
N_{ij}&=& p_l\lambda_j T_{ij} \\
&=& \frac{p_l\lambda_j K}{\Lambda_i}
\end{eqnarray}

  This concludes the proof
\end{proof}


==> relatedworkcomments.tex <==
abebe2017fair

@inproceedings{abebe2017fair,
  title={Fair division via social comparison},
  author={Abebe, Rediet and Kleinberg, Jon and Parkes, David C},
  booktitle={Proceedings of the 16th Conference on Autonomous Agents and MultiAgent Systems},
  pages={281--289},
  year={2017},
  organization={International Foundation for Autonomous Agents and Multiagent Systems}
}


this paper discusses solutions to the cake cutting problem

non-parametric: the authors only need to compare utilities, but they do not need to take derivatives of utilities. The authors do not rely on the shape of the utility functions to derive any results.  The authors only need to assume that valuation functions are additive, non-atomic, and non-negative. 


zhangfairness


@article{zhangfairness,
  title={Fairness in Decision-Making: The Causal Explanation Formula},
  author={Zhang, Junzhe and Bareinboim, Elias},
  year={2017},
  journal={Purdue technical report R-30-L}
}


causality work

non-parametric: works on causality usually do not consider parametric shapes for utilities or distributions 






the classifiers considered are parametric, and target maximizing true positive and true negative raets, and equalizing false positive and false negative rates

or, in classification problems, cost functions which are linear combinations of false positive and false negative rates

kleinberg2016inherent

@article{kleinberg2016inherent,
  title={Inherent trade-offs in the fair determination of risk scores},
  author={Kleinberg, Jon and Mullainathan, Sendhil and Raghavan, Manish},
  journal={arXiv preprint arXiv:1609.05807},
  year={2016}
}

pleiss2017fairness

@inproceedings{pleiss2017fairness,
  title={On fairness and calibration},
  author={Pleiss, Geoff and Raghavan, Manish and Wu, Felix and Kleinberg, Jon and Weinberger, Kilian Q},
  booktitle={Advances in Neural Information Processing Systems},
  pages={5684--5693},
  year={2017}
}




corbett2017algorithmic


@inproceedings{corbett2017algorithmic,
  title={Algorithmic decision making and the cost of fairness},
  author={Corbett-Davies, Sam and Pierson, Emma and Feller, Avi and Goel, Sharad and Huq, Aziz},
  booktitle={Proceedings of the 23rd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
  pages={797--806},
  year={2017},
  organization={ACM}
}



